Adversarial Transfer of Pose Estimation Regression

We address the problem of camera pose estimation in visual localization. Current regression-based methods for pose estimation are trained and evaluated scene-wise. They depend on the coordinate frame of the training dataset and show a low generalization across scenes and datasets. We identify the dataset shift an important barrier to generalization and consider transfer learning as an alternative way towards a better reuse of pose estimation models. We revise domain adaptation techniques for classification and extend them to camera pose estimation, which is a multi-regression task. We develop a deep adaptation network for learning scene-invariant image representations and use adversarial learning to generate such representations for model transfer. We enrich the network with self-supervised learning and use the adaptability theory to validate the existence of scene-invariant representation of images in two given scenes. We evaluate our network on two public datasets, Cambridge Landmarks and 7Scene, demonstrate its superiority over several baselines and compare to the state of the art methods.

==> cambridge-da.tex <==
\begin{table*}[ht]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{||l|l||r|r|r|r||} \hline
Dataset	 & Method  & Old      & King    & StMary & Shop    \\ \hline
%         & Ratio   & Hospital & College & Church & Facade  \\ \hline

Old    &Transposed      & &    14.04/22.12&    21.81/47.22 &   22.12/36.33 \\ 
\cline{2-2} \cline{4-6}
       & Joint          & &{\it 1.46/4.78}& {\it 2.30/7.46} &{\it 2.51/7.53} \\ 
\cline{2-2} \cline{4-6}
       & SS,  $\nu$=0.05& &     7.36/14.03&     7.24/12.19 &     6.47/13.71 \\
       & APANet,$\nu$=0.05& &{\bf 4.21/6.83}&{\bf 3.82/9.54} &{\bf 3.56/9.37} \\ 
\hline
Kings  &Transposed      &12.77/15.31 & & 17.09/44.02 & 8.17/21.62 \\ 
\cline{2-3} \cline{5-6}
       & Joint          &{\it 1.55/5.05}& &{\it  2.19/6.65} &{\it 1.32/4.58} \\
\cline{2-3} \cline{5-6}
       & SS,  $\nu$=0.05&     6.74/14.92& &     6.76/15.84 &     6.52/13.10 \\
       & APANet,$\nu$=0.05&{\bf 3.74/8.27}& &{\bf 3.88/10.18}&{\bf 2.61/8.63} \\ 
\hline            
StMarys&Transposed      &     12.34/22.01&  11.96/17.32& &      10.13/23.21 \\ \cline{2-4} \cline{6-6}
       & Joint          &{\it 2.40/7.80} &{\it 2.23/6.85} & & {\it 2.05/7.70} \\ \cline{2-4} \cline{6-6}
       & SS,  $\nu$=0.05&     7.18/19.00 &     7.07/14.37& &     5.95/13.44 \\
       & APANet,$\nu$=0.05&{\bf 4.84/11.30}&{\bf 4.00/8.11}& &{\bf 3.92/9.25}\\ 
\hline
Shop   &Transposed      &    12.64/19.76 &   15.49/21.08  & 20.39/51.37 & \\\cline{2-5}
       & Joint          &{\it 2.46/7.69 }&{\it 1.49/5.91} &{\it 2.13/7.65} & \\\cline{2-5}  
       & SS,  $\nu$=0.05&     8.12/15.91 &    7.64/13.00  & 6.83/17.41 & \\
       & APANet,$\nu$=0.05&{\bf 3.64/10.19}&{\bf 3.84/8.40} & {\bf 3.73/10.64} & \\ 
\hline
\end{tabular}}
\caption{Pose adaptation in Cambridge Landmarks dataset. We report the median position (in meters) / orientation (in degrees) errors.}
\end{center}
\label{tab:cambridge}
\end{table*}

==> contribution-ip.tex <==

\subsection{Contribution (Preliminary Claims}
%=========================================================
The main contributions of this paper are the following:
\begin{enumerate}

\item 
We address the problem of weak generalization of the camera pose estimation models,
%Known for low generalization, the deep methods for absolute pose estimation. 
when directly regressing the absolute camera pose (APR) constrains the machine learning models to be trained and evaluated scene-wise.
%when the scenes are registered to different coordinate frames. 
%The reason for this is that 
%The trained model learns a mapping from image to pose which is dependent on the coordinate frame of the training data. % belonging to a particular scene. %This 
%causes complications, especially if one is interested in localization across several scenes simultaneously, and also 
%This prevents transferring learned knowledge of geometric relations between scenes.
We propose adaptation across scenes as an alternative way towards a better generalization of APR models.

\item  
We extend domain adaptation techniques for classification to the multi-regression task and developed a deep network to adapt a pose regression model from one scene to another. 
 
\item 
We develop the Adversarial Pose Adaptation Network (APANet) to learn scene-invariant image representations and to use target scene supplements to guide the adaptation of source APR model to the target scene.
 
\item
We implement pose-driven and aggregation-based approaches to guide the transfer, based on the aggregated information about the target scene. This knowledge may accompany the unsupervised adaptation of the pose regressor from one domain to another.

%\item
%A regression model can be adopted to a target scene and new reference with a rather small annotation effort with our explicit transformation between the domains and coordination systems.
%tiny annotation part as little as few percents of data
%\item 
%Weak target scene annotation guides the transfer towards  the range and scale of target poses.
%Semi-supervised adaptation is only one of possible ways to adapt regressors. In the difference from unsupervised domain adaptation in the classification task challenges due to the complex topology.

\item 
We also apply the adaptability theory to validate the existence of domain-invariant representation of images in two scenes and to measure the transferability of feature representations from one scene to another.

\item 
We validate the advantages of the APANet over the baselines on Cambridge Landmarks and 7Scene datasets.
\end{enumerate}



==> table-scene_overlap.tex <==
%Dataset bias in relative poses 
%In test of source test set, 
%percentage of 1-top neigbour being in Trg train set

%> python test_ktrees.py

%1-to-1 in Cambridge , Source to Target

%0 1 Pos= [26] Neg= [155] Ratio= 0.143646408839779
%0 2 Pos= [74] Neg= [107] Ratio= 0.4088397790055249
%0 3 Pos= [12] Neg= [169] Ratio= 0.06629834254143646
%1 0 Pos= [30] Neg= [312] Ratio= 0.08771929824561403
%1 2 Pos= [43] Neg= [299] Ratio= 0.12573099415204678
%1 3 Pos= [34] Neg= [308] Ratio= 0.09941520467836257
%2 0 Pos= [99] Neg= [431] Ratio= 0.18679245283018867
%2 1 Pos= [57] Neg= [473] Ratio= 0.10754716981132076
%2 3 Pos= [9] Neg= [521] Ratio= 0.016981132075471698
%3 0 Pos= [18] Neg= [85] Ratio= 0.17475728155339806
%3 1 Pos= [64] Neg= [39] Ratio= 0.6213592233009708
%3 2 Pos= [15] Neg= [88] Ratio= 0.14563106796116504

%3 to 1 in Cambridge
%Tr Src: (894, 6) Te Src: (181, 6) Tr Trg: (2937, 6) Te Trg: (975, 6)
%0 Pos= [82] Neg= [99] Ratio= 0.4530386740331492
%Tr Src: (1219, 6) Te Src: (342, 6) Tr Trg: (2612, 6) Te Trg: (814, 6)
%1 Pos= [77] Neg= [265] Ratio= 0.22514619883040934
%Tr Src: (1487, 6) Te Src: (530, 6) Tr Trg: (2344, 6) Te Trg: (626, 6)
%2 Pos= [139] Neg= [391] Ratio= 0.2622641509433962
%Tr Src: (231, 6) Te Src: (103, 6) Tr Trg: (3600, 6) Te Trg: (1053, 6)
%3 Pos= [65] Neg= [38] Ratio= 0.6310679611650486

\begin{table}[ht]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{|lrrrr} \hline
Source & Kings &Old  & StMarys& Shop \\ \hline
Kings  &       &8.7  & 30.1   & 6.6 \\ 
Old    &14.3   &     &    12.5& 9.9 \\ 
StMarys&18.6   &10.7 &        & 1.7 \\ 
Shop   & 17.4  & 52.1& 14.5   &     \\
\end{tabular}}
\end{center}
\end{table}

